Benchmarking Long-tail Generalization with Likelihood Splits

In order to reliably process natural language, NLP systems must generalize to the long tail of rare utterances. We propose a method to create challenging benchmarks that require generalizing to the tail of the distribution by re-splitting existing datasets. We create 'Likelihood Splits' where examples that are assigned lower likelihood by a pre-trained language model (LM) are placed in the test set, and more likely examples are in the training set. This simple approach can be customized to construct meaningful train-test splits for a wide range of tasks. Likelihood Splits surface more challenges than random splits: relative error rates of state-of-the-art models increase by 59% for semantic parsing on Spider, 93% for natural language inference on SNLI, and 33% for yes/no question answering on BoolQ, on our splits compared with the corresponding random splits. Moreover, Likelihood Splits create fairer benchmarks than adversarial filtering; when the LM used to create the splits is also employed as the task model, our splits do not unfairly penalize the LM.

==> scratch_space.tex <==
%%%
% Abstract
%%%

% We \textit{will attempt} to show that the language model score highlights the \textit{tail} of the distribution within existing curated datasets.

% We \textit{hope to} demonstrate methods to tackle out-of-distribution (OOD) generalization are required to overcome this challenging split and that 
% By the nature of the data distribution, standard dataset curation strategies tend to over-sample the \textit{head} of the distribution while under-sampling the \textit{tail} of the distribution. This leads to models that learn strategies to solve the data-rich head of the distribution and ignore the complexity involved in generalizing to the tail of the distribution. At the same time, curating a dataset that samples explicitly from the tail of the distribution is an ill-posed problem: annotators would be required to ask unnatural queries. In this work, we propose to use a pre-trained language model to highlight the \textit{tail} of the distribution within existing curated datasets. We primarily focus on the task of semantic parsing and explore the properties of the dataset splits created by our strategy. We further extend some of the analysis to text classification datasets. We demonstrate that our proposed splits naturally contain a mixture of several generalization challenges that have been studied separately in the past.

%%%
% Intro
%%%

% In this work, we propose a method to generate an out-of-distribution generalization challenge that harnesses a natural source of difficulty: the heavy-tailed Zipfian distribution \citep{10.2307/2572028-zipf} of language. It has been shown for multiple languages that there are a large number of utterances individually that occur very rarely, but together contribute to a large portion of the usage of language. We posit that the challenge of generalizing to rare cases requires models to demonstrate a wide variety of skills which are important for understanding language in general; benchmarks that pose the task of generalizing from the likely utterances to the unlikely utterances are a valuable axis to evaluate model performance.

% By the very nature of the long-tail, it is impossible to exhaustively sample data points that cover all infrequent phenomena. Additionally, the current tools for dataset curation such as Amazon Mechanical Turk (and similar services that offer access to a huge pool of annotators at a cost) cannot be directly employed to sample from the tail. This would require the creation of annotation guidelines for the ill-defined problem of generating ``rare" queries. 
% Instead, we focus on trying to capture the tail of the distribution within existing datasets. We approximately capture this tail using the likelihood under a large, pre-trained language-model \gpt \citep{radford2019language-gpt2}. These models are exposed to vast amounts of text during their pre-training phase and trained under the empirical risk minimization framework coupled with the language modelling objective, which aims to increase the likelihood of text weighted by the empirical probability of seeing the text. We believe that this should enable models to assign the low-frequency, tail utterances a lower likelihood than the high-frequency head of the distribution. Thus, we instantiate long-tail generalization benchmarks that require models to train on the head of the distribution and generalize to the tail (see Fig \ref{fig:method-eye-candy}).

% Our proposed method is \emph{widely-applicable} and can be easily extended to a range of language tasks at no additional annotation cost. The resulting generalization benchmarks that are more \emph{challenging} than the standard IID (random) splits. We demonstrate this by creating \textbf{Likelihood splits} for the task of semantic parsing on the \spider dataset \citep{yu-etal-2018-spider},
% % (since it has been used as a setting for creating \emph{challenge} data splits previously) and 
% natural language inference (NLI) on the \snli dataset \citep{bowman-etal-2015-large-snli},
% % (since it has been the focus of several dataset curation studies).
% and yes/no question answering on the \boolq dataset \citep{clark-etal-2019-boolq}. The resulting data split is agnostic to the task models and is \emph{not designed to be adversarial} to a particular model class or training algorithm.
% % Unlike in-distribution benchmarks, this split poses the challenge of generalizing to rare cases.
% % and avoid some of the pitfalls of collecting adversarial examples \citep{arxiv.2111.08181-unfair-adversarial}.
% We do not aim to isolate any particular linguistic or reasoning skill; however, we show that to perform well on the proposed split, a model \emph{needs to demonstrate a mixture of skills}, systematic compositional generalization, and handling more complex language. Given the relative ease of applying our proposed approach, we encourage future benchmarks to create and release \emph{Likelihood splits} as complementary evaluation to the standard IID evaluation as means to better test out-of-distribution generalization performance of competing models.

% Our analysis will be focused on the task of semantic parsing (since it has been used as a setting for creating \emph{challenge} data splits previously) and natural language inference (NLI) (since it has been the focus of several dataset curation studies). For semantic parsing, we will describe the properties studied by past work in creating these splits and show that they also appear in our proposed data split. \robin{< Too vague, either be specific or omit} For both settings, we make attempts to uncover the source of the difficulty. \robin{< Should say what the key difficulties are.} We hope to establish our split as a natural out-of-distribution (OOD) generalization challenge. \robin{< Too modest. Maybe be more direct and say something like, we encourage new benchmarks to include likelihood splits as a standard evaluation setting.} Our proposed method is simple, applicable to a wide variety of tasks, and can be used to create interesting generalization benchmarks at no additional annotation cost.

%%%
% Related work
%%%

% \subsection{Model design and training}
% Several dataset specific approaches have been developed to tackle the challenges posed by synthetic datasets \citep{liu2020-scan-generalization,li-etal-2019-compositional-scan-generalization}. Intriguingly, some of these approaches tend to perform well only on certain splits of the datasets. More general studies of model properties that improve generalization include \citep{russin2019-composition-separation,Gordon2020Permutation,dessi-baroni-2019-cnns}. With each of the datasets mentioned in the previous section, authors have shown that existing modelling techniques cannot perform the expected generalization. In particular, most prior work demonstrated surprisingly poor performance of \emph{Transformer} based models which have otherwise dominated NLP tasks. These claims were challenged by \cite{csordas2021-devil-in-detail} who showed that certain design decisions such as using relative positional embeddings \cite{dai-etal-2019-transformerxl}, scaling of input embeddings and longer training allow \emph{Transformer}s to excel at these generalization tasks.

% Data augmentation techniques such as \citep{andreas-2020-geca,akyurek2021-comp-augmentation,oren2021-comp-augmentation-needles} improve generalization by training on generated data which contains novel compositions of existing training data. Meta-learning provides an exciting approach to incentivize generalization in model training by creating meta-test sets that are systematically diverse from the meta-train set \citep{lake2019-comp-meta,conklin-etal-2021-comp-meta}.

% Most works test the performance of models trained from scratch on these challenge datasets. To the best of our knowledge, \cite{furrer2020-pretrain-compositional} is the only study of the performance of pre-trained language models on compositional generalization benchmarks. They evaluate pre-trained T5 \cite{raffel2020-t5} model variants fine-tuned on SCAN and CFQ, and find gains over non-pretrained variants of the same model. The benefit from using a pre-trained language model mainly comes from being able to handle substitutions of similar words and phrases. But pre-training does not lead to globally better performance over other methods.

% \subsection{Effect of model modification on external datasets}
% Most of the methods discussed in the previous section show improvement only in synthetic datasets that they were designed for. The results in these works don’t show whether getting better at these tasks is a useful for downstream task performance. Some exceptions include: \cite{shaw-etal-2021-compositional-tmcd} report performance gains on \textsc{Spider} and \textsc{GeoQuery} datasets; \cite{andreas-2020-geca} which report improved performance on \textsc{GeoQuery} semantic parsing tasks. 

% One of the draws of studying systematic generalization is the (human-like ability) to generalize from a small amount of data to an infinite number of novel utterances (``make infinite use of finite means"). This would be a useful feature for data scarce tasks such as low-resource learning and few-shot learning. \cite{andreas-2020-geca} showed that their data augmentation techniques could be successfully transferred for modest improvements in low-resource language modelling.

% \cite{chaabouni2021-jump-transformers} conducted a systematic analysis of model modifications that can be carried over from Convolutional Seq2Seq \cite{dessi-baroni-2019-cnns} models to \textit{Transformers} for improved performance on SCAN. They train these modified \textit{Transformers} on a English-German (high-resource) machine translation task and discard the modifications that hurt MT performance. Finally, they show that these modifications lead to improvement in low-resource machine translation (English-Sinhala and English-Nepali).

% \citet{sogaard-etal-2021-need-to-talk-about-random-splits} argue that the standard methodology of dataset collection does not accurately predict the model performance on \textit{new in-domain} data. In particular, they evaluate performance of state-of-the-art models for 7 NLP tasks (part-of-speech tagging, sentence representation probing (2 tasks), translation quality estimation, headline generation, emoji prediction and new classification) on several splits of the dataset (standard, random, length heuristic-based, adversarial and new in-domain9). The model performance on new samples drawn from the same domain (temporal split if allowed by the dataset) is over-estimated by random and standard splits. Heuristic and adversarial splits sometimes over-estimate in-domain performance. As a guideline, the authors propose the use of new samples if available or to generate multiple biased splits to better estimate real-world performance. Our work is another attempt in this direction but it does not involve any human engineering in defining the types of bias and isolating it. However, our method of creating likelihood based data splits also introduces a distribution shift (from training on the head to predicting on the tail) which needs to be addressed when designing models and training algorithms.

% \citet{LeBras2020AdversarialFilters} provide a method for automatically detecting and removing samples that induce bias towards spurious features. They show that while their dataset pruning leads to reduced in-domain performance (which is a well-known phenomena in bias reduction), they see improved out-of-domain generalization in both NLP and vision tasks. It should be noted that removing bias in trained models is not the focus of our work. Similarly, we haven't explored how to handle the out-of-distribution generalization problem created by our split generation procedure. However, in order to motivate the usefulness of the approach, it would be interesting to check whether model selection based on our proposed data split leads to similar improvements in out-of-domain generalization.

% The general practice in model development on a dataset involves the use of a \textit{standard/random split}. \citet{sogaard-etal-2021-need-to-talk-about-random-splits} challenge the utility of these splits in predicting performance on new data drawn from the same domain by showing that they often over-estimate in-domain performance. In response to these observations, there has been a lot of work on filtering datasets to remove examples that induce bias \citep{LeBras2020AdversarialFilters}, and creating splits that put the  challenging queries in the evaluation sets \citep{yang2018hotpotqa, potts-etal-2021-dynasent}. Similarly, certain data splits are designed to isolate and study linguistic skills: length-generalization \citep{SCAN-dataset}, compositional generalization \citep{SCAN-dataset, COGS-Dataset, CFQ-Dataset, shaw-etal-2021-compositional-tmcd, gu2021beyond-grailqa}, domain generalization \citep{yu-etal-2018-spider, gu2021beyond-grailqa}.

%%%
% \subsection{Text Classification}
%%%

% Text classification is the task of predicting a categorical label given an input sentence. In this work, we focus on sentiment analysis, which is the task of predicting whether a particular statement conveys positive, neutral or negative sentiment (with varying levels) about some subject being considered. We will study split properties on movie reviews in the \textsc{IMDB} dataset \citep{10.5555/2002472.2002491-imdb} (2-way classification) and \textsc{SST} \citep{socher-etal-2013-recursive-sst5} (5-way classification). For both datasets, the evaluation metric considered will be the average accuracy (since classes are relatively balanced).

%%%
% Original results with GPT2-large splits on just train_spider
%%%

% \begin{table}[bt]
% \centering
% \begin{tabular}{| l | c |}
% \hline
% \textbf{Split} & \textbf{Spider}\\
% \hline
% Standard & 75.2\\
% Length & 40.7\\
% Template & 47.8\\
% TMCD & 49.8\\
% \hline
% * TMCD (CD=0.041) & 73.66\\
% \hline
% ll\_split & 55.7\\
% ll\_split (-length) & 59.8 \\
% \hline
% ll\_split prompt & 58.0\\
% ll\_split prompt (-length) & 66.5 \\
% \hline
% \end{tabular}
% \caption{\label{tab:parsing-acc}
% Exact sequence prediction accuracy of the semantic parsing task on \textsc{Spider} for various splits. \emph{Template} refers to \cite{finegan-dollak-etal-2018-improving}. \emph{TMCD} refers to \cite{shaw-etal-2021-compositional-tmcd}. NOTE: TMCD (CD=0.041) is a version of the TMCD algorithm which is stopped at the level of compound divergence demonstrated by the likelihood splits.}
% \end{table}

%%%
% Methodology
%%%

% In recent years, large neural network models have been trained with language modelling objectives on text gathered from varied sources on the internet \citep{devlin-etal-2019-bert,dai-etal-2019-transformerxl,raffel2020-t5}. Some of these retain the left-to-right causal language modelling framework \citep{radford2019language-gpt2}. We make the assumption that the tail of the true data distribution is captured by the likelihood under a trained language model (LM). Different from prior work, this allows us to create a dataset split which is not designed based on human intuition or domain insights, and hence the approach is easy to apply to a range of tasks. Moreover, it is not adversarial to any particular model class since the partitioning is task-model agnostic.

% We propose two approaches to define and capture the tail of the distribution. If the dataset curator aims to capture phenomena that are under-represented in the specific collected data, then it might be preferable to fine-tune the language model on the gathered data (\S\ref{sec:gpt-ft-setup}) since it would better capture the language distribution for the task. If the phenomena to be captured are under-represented in the general use of language, then it might be preferable to use the pre-trained language model without further fine-tuning (\S\ref{sec:gpt-prompt-setup}), since it would better capture the frequency of utterances in the wild.

%%%
% Rare words
%%%

% Template split does not promote language variation. The test set of the TMCD split contains a greater fraction of the rare words than the mean but within the variation of random splits. However, since it selects shorter utterances, a larger fraction of the test set words are rare. The length split, and in turn longer queries, seems to be directly correlated with rare words i.e. the rare words are more likely to occur in longer utterances. As a result, the likelihood splits (which also puts longer queries in the test set) seem to have a language variation that is significantly different from the random split. When we check fraction of the test set words that are rare, the distribution of the length split is within the variation of the null statistic. Fine-tuning reduces the surprise of the language model to rare words that occur in the dataset as compared to a prompted language model i.e. the challenge of generalizing to rare words is less severe when using a fine-tuned language model.

% \begin{figure}[tb]
% \centering
% \begin{subfigure}{0.48\textwidth}
% \centering
% \includegraphics[width=\textwidth]{images/spider-word-stats (1).png}
% \caption{All likelihood based splits retain a larger fraction of the utterances with the rare word in the test set. Since the length split also shows a large fraction of rare words, it shows that rare words are more likely to appear in longer utterances.}
% \end{subfigure}

% \begin{subfigure}{0.48\textwidth}
% \centering
% \includegraphics[width=\textwidth]{images/spider-word-stats (2).png}
% \caption{We demonstrate that longer utterances contain rare words by checking what fraction of test set words are rare. When not controlling for length, likelihood based splits put utterance with rare words in the test set.}
% \end{subfigure}

% \caption{Various statistics of the rare words in the test set of various splits (on the \textsc{Spider} dataset). This is plotted against the distribution of values observed for 500 random slits of the data. ll\_split variants retain rare words in the test set. Fine-tuning to the dataset, reduces the "surprise" of the language model to the rare words in the dataset.}
% \label{fig:spider-rare-test-words}
% \end{figure}

%%%
% SNLI BOOLQ tables
%%%

% \begin{table*}[tb]
% \centering
% \footnotesize
% \begin{tabular}{ l c c c c c }
% \hline
%  & \multirow{2}{*}{Random} & \multicolumn{2}{c}{ll\_split} & \multicolumn{2}{c}{ll\_split pt} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
% System & & & (-len) & & (-len) \\
% \hline
% \roberta-base & 89.6 \scriptsize{$\pm$0.38} & 78.41 & 75.01 & 82.61 & 81.71 \\
% \roberta-large & 90.53 \scriptsize{$\pm$0.48}  & 82.06 & 79.00 & 85.01 & 84.25 \\
% \electra-base & 90.49 \scriptsize{$\pm$0.17} & 80.13 & 77.6 & 82.86 & 82.8 \\
% \electra-large & 90.96 \scriptsize{$\pm$1.33} & 84.04 & 80.59 & 85.92 & 84.86 \\
% \hline
% \roberta-large & 70.18 \scriptsize{$\pm$0.29} & 62.91 & 62.75 & 67.18 & 69.55 \\
% \textit{(Hypothesis only)} \\
% \hline
% Human Accuracy & 88.74 \scriptsize{$\pm$0.8} & 83.04 & 84.00 & 85.24 & 86.38 \\
% \hline
% \end{tabular}
% \caption{\label{tab:snli-acc}
% Accuracy on the NLI task on \snli for various splits and model sizes. Likelihood splits lead to decreased model performance. The performance gap between two model sizes in the same model class are wider on our proposed splits.}
% \end{table*}

% \begin{table*}[tb]
% \centering
% \begin{tabular}{ l c c c c c }
% \hline
%  & \multirow{2}{*}{Random} & \multicolumn{2}{c}{ll\_split} & \multicolumn{2}{c}{ll\_split prompt} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6}
% System & & & (-length) & & (-length) \\
% \hline
% \roberta-base & 74.94 \small{$\pm$0.36} & 71.14 & 70.31 & 72.4 & 71.89 \\
% \roberta-large & 84.37 \small{$\pm$0.62} & 78.43 & 78.27 & 82.28 & 80.59 \\
% \electra-base & 78.78 \small{$\pm$1.11} & 75.04 & 73.9 & 75.24 & 73.58 \\
% \electra-large & 85.46 \small{$\pm$0.62} & 82.99 & 80.59 & 83.7 & 81.85 \\
% \hline
% \end{tabular}
% \caption{\label{tab:boolq-acc}
% Accuracy on the \textsc{BoolQ} question answering task various splits and model sizes. Likelihood based splits lead to decreased model performance compared to random splits. Removing the factor of length increases the difficulty of Likelihood splits.}
% \end{table*}

% \begin{table*}[tb]
% \centering
% \footnotesize
% \begin{tabular}{ l c c c c c c c c c c}
% \toprule
% & \multicolumn{5}{c}{\textbf{\snli}} & \multicolumn{5}{c}{\textbf{\boolq}}\\
% \cmidrule(lr){2-6} \cmidrule(lr){7-11}
%  & \multirow{2}{*}{Random} & \multicolumn{2}{c}{ll\_split} & \multicolumn{2}{c}{ll\_split pt} & \multirow{2}{*}{Random} & \multicolumn{2}{c}{ll\_split} & \multicolumn{2}{c}{ll\_split pt} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
% \textbf{System} & & & (-len) & & (-len) & & & (-len) & & (-len) \\
% \midrule[\heavyrulewidth]
% \roberta-base & 89.6 \scriptsize{$\pm$0.38} & 78.41 & 75.01 & 82.61 & 81.71 & 74.94 \scriptsize{$\pm$0.36} & 71.14 & 70.31 & 72.4 & 71.89 \\
% \roberta-large & 90.53 \scriptsize{$\pm$0.48}  & 82.06 & 79.00 & 85.01 & 84.25 & 84.37 \scriptsize{$\pm$0.62} & 78.43 & 78.27 & 82.28 & 80.59 \\
% \electra-base & 90.49 \scriptsize{$\pm$0.17} & 80.13 & 77.6 & 82.86 & 82.8 & 78.78 \scriptsize{$\pm$1.11} & 75.04 & 73.9 & 75.24 & 73.58 \\
% \electra-large & 90.96 \scriptsize{$\pm$1.33} & 84.04 & 80.59 & 85.92 & 84.86 & 85.46 \scriptsize{$\pm$0.62} & 82.99 & 80.59 & 83.7 & 81.85 \\
% \midrule[\heavyrulewidth]
% R-large Hyp.-only & 70.18 \scriptsize{$\pm$0.29} & 62.91 & 62.75 & 67.18 & 69.55 & - & - & - & - & - \\
% %\textit{(Hypothesis only)} \\
% \midrule
% Human Accuracy & 88.74 \scriptsize{$\pm$0.8} & 83.04 & 84.00 & 85.24 & 86.38 & - & - & - & - & - \\
% \bottomrule
% \end{tabular}
% \caption{\label{tab:snli-acc}
% Accuracy on \snli and \boolq for various splits and model sizes. Likelihood splits lead to decreased model performance. Controlling for length further increases the difficulty.}
% \end{table*}
